New quasar proximity zone size measurements at $z\sim 6$ using the enlarged XQR-30 sample

Proximity zones of high-redshift quasars are unique probes of their central supermassive black holes as well as the intergalactic medium in the last stages of reionization. We present 22 new measurements of proximity zones of quasars with redshifts between 5.8 and 6.6, using the enlarged XQR-30 sample of high-resolution, high-SNR quasar spectra. The quasars in our sample have UV magnitudes of $M_{1450}\sim -27$ and black hole masses of $10^9$$\unicode{x2013}$$10^{10}$ M$_\odot$. Our inferred proximity zone sizes are 2$\unicode{x2013}$7 physical Mpc, with a typical uncertainty of less than 0.5 physical Mpc, which, for the first time, also includes uncertainty in the quasar continuum. We find that the correlation between proximity zone sizes and the quasar redshift, luminosity, or black hole mass, indicates a large diversity of quasar lifetimes. Two of our proximity zone sizes are exceptionally small. The spectrum of one of these quasars, with $z=6.02$, displays, unusually for this redshift, damping wing absorption without any detectable metal lines, which could potentially originate from the IGM. The other quasar has a high-ionization absorber $\sim$0.5 pMpc from the edge of the proximity zone. This work increases the number of proximity zone measurements available in the last stages of cosmic reionization to 87. This data will lead to better constraints on quasar lifetimes and obscuration fractions at high redshift, which in turn will help probe the seed mass and formation redshift of supermassive black holes.

==> main_table.tex <==
%% DO NOT DELETE the table even if it's not needed in the paper.
\begin{comment}
  \begin{center}
    \begin{table*}
      \centering
      \begin{tabular} {p{0.05\textwidth} p{0.15\textwidth} p{0.15\textwidth}  p{0.05\textwidth} p{0.1\textwidth} p{0.15\textwidth} p{0.15\textwidth}p{0.05\textwidth}}
        \hline
        \hline 
        S.~N.\ & Object & $z_\mathrm{qso}$  & Line & $M_{1450}$ & $\rp$ & $\rpc$  &Refs.\\
        &          &              &              &     & (pMpc)  & (pMpc) \\
        \hline
        1 & J0408-5632  & $6.033^{\scaleto{+0.0107}{4pt}}_{\scaleto{-0.006}{4pt}}$& \MgII & $-26.56$& $3.00^{\scaleto{+0.66}{4pt}}_{\scaleto{-0.37}{4pt}}$ &$3.5^{\scaleto{+0.76}{4pt}}_{\scaleto{-0.43}{4pt}}$ &(1,-) \\ 
        2 & PSOJ029-29 & $5.976^{+\scaleto{+0.0106}{4pt}}_{\scaleto{-0.006}{4pt}}$ & \MgII & $-27.32$& $4.91^{\scaleto{+0.66}{4pt}}_{\scaleto{-0.37}{4pt}}$ &$4.4^{\scaleto{+0.59}{4pt}}_{\scaleto{-0.33}{4pt}}$&(1,9) \\ 
        3 & ATLASJ029-36 & $ 6.013^{\scaleto{+0.0106}{4pt}}_{\scaleto{-0.006}{4pt}}$ & \MgII &  $-27.0$ &$4.33^{\scaleto{+0.65}{4pt}}_{\scaleto{-0.37}{4pt}}$&$4.34^{\scaleto{+0.65}{4pt}}_{\scaleto{-0.37}{4pt}}$ &(1,9)\\
        4 & VDESJ0224-4711 & $6.525^{\scaleto{+0.0114}{4pt}}_{\scaleto{-0.0064}{4pt}}$  & \MgII & $-26.93$&$6.45^{\scaleto{+0.59}{4pt}}_{\scaleto{-0.35}{4pt}}$&$6.61^{\scaleto{+0.6}{4pt}}_{\scaleto{-0.35}{4pt}}$ &(1,10)\\
        5 & PSOJ060+24 & $6.17^{\scaleto{+0.0109}{4pt}}_{\scaleto{-0.0061}{4pt}}$  & \MgII & $-26.95$&$4.13^{\scaleto{+0.63}{4pt}}_{\scaleto{-0.35}{4pt}}$&$4.2^{\scaleto{+0.65}{4pt}}_{\scaleto{-0.36}{4pt}}$ &(1,9)\\
        6 & PSOJ108+08 & 5.9647$\pm$0.0023  &  \CII & $-27.59$ &$1.99^{\scaleto{+0.14}{4pt}}_{\scaleto{-0.46}{4pt}}$&$1.63^{\scaleto{+0.12}{4pt}}_{\scaleto{-0.37}{4pt}}$&(-,9)\\
        7 & SDSSJ0842+1218 & 6.0754$\pm$ 0.0024 &  \CII &$-26.91$& 6.89$\pm$0.14& 7.11$\pm$0.15&(2,9)\\
        8 & PSOJ158-14 & 6.0687$\pm$   0.0024 &  \CII&$-27.51$& 1.95$\pm$0.14&1.63$\pm$0.12&(-,-)\\
        9 & PSOJ183-12 &  $5.86^{\scaleto{+0.0104}{4pt}}_{\scaleto{-0.0059}{4pt}}$  & \MgII & $-27.49$&$3.06^{\scaleto{+0.67}{4pt}}_{\scaleto{-0.38}{4pt}}$&$2.58^{\scaleto{+0.57}{4pt}}_{\scaleto{-0.32}{4pt}}$ &(9,9)\\
        10& PSOJ217-16 &  6.1466$\pm$ 0.0024 &  \CII & $-26.94$&$2.88^{\scaleto{+0.14}{4pt}}_{\scaleto{-0.6}{4pt}}$&$2.94^{\scaleto{+0.14}{4pt}}_{\scaleto{-0.61}{4pt}}$ &(-,9)\\
        11& PSOJ242-12 & 5.8468$\pm$ 0.0023 &  \CII & $-26.92$&4.87$\pm$0.15&5.01$\pm$0.15 &(-,9)\\
        12& PSOJ308-27 & $5.799^{\scaleto{+0.0103}{4pt}}_{\scaleto{-0.0058}{4pt}}$  & \MgII & $-26.78$ &$2.95^{\scaleto{+0.68}{4pt}}_{\scaleto{-0.38}{4pt}}$&$3.19^{\scaleto{+0.74}{4pt}}_{\scaleto{-0.41}{4pt}}$ &(-,9)\\
        13& PSOJ323+12 & 6.5872$\pm$0.0025 & \CII & $-27.12$ &6.2$\pm$0.13&5.95$\pm$0.12 &(2,-)\\
        14& PSOJ359-06 & 6.1719$\pm$ 0.0024 & \CII & $-26.79$ &2.71$\pm$0.14&2.92$\pm$ 0.15&(2,9)\\
        15& SDSSJ0927+2001 & 5.7722$\pm$0.0023 & CO &$-26.76$&4.7$\pm$0.15&5.1 $\pm$0.16&(3,9)\\
        16& SDSSJ0818+1722 & 6.02$\pm$0.0234 &\lya&$-27.52$&$5.13^{\scaleto{+1.43}{4pt}}_{\scaleto{-2.35}{4pt}}$ &$4.29^{\scaleto{+1.2}{4pt}}_{\scaleto{-1.96}{4pt}}$&(4,9)\\
        17& SDSSJ1306+0356 & 6.033$\pm$0.0023&\CII&$-27.1$& $6.43^{\scaleto{+0.14}{4pt}}_{\scaleto{-0.15}{4pt}}$&6.21$\pm$0.14&(5,11)\\
        18& ULASJ1319+0950 & 6.1347$\pm$0.0024 &\CII&$-27.05$& $3.87^{\scaleto{+1.08}{4pt}}_{\scaleto{-0.14}{4pt}}$&$3.81^{\scaleto{+1.07}{4pt}}_{\scaleto{-0.14}{4pt}}$&(6,9)\\
        19& SDSSJ1030+0524 &$ 6.309^{\scaleto{+0.0111}{4pt}}_{\scaleto{-0.0062}{4pt}}$ &\MgII&$-26.99$&$5.47^{\scaleto{+0.61}{4pt}}_{\scaleto{-0.34}{4pt}}$&$5.49^{\scaleto{+0.61}{4pt}}_{\scaleto{-0.35}{4pt}}$&(7,9)\\
        20& SDSSJ0100+2802&6.3269$\pm$0.0024&\CII&$-29.14$&$7.22^{\scaleto{+0.13}{4pt}}_{\scaleto{-0.14}{4pt}}$&$3.43^{\scaleto{+0.06}{4pt}}_{\scaleto{-0.07}{4pt}}$&(8,9)\\
        21& ATLASJ025-33&6.3373$\pm$0.0024 &\CII&$-27.5$&$6.5^{\scaleto{+0.14}{4pt}}_{\scaleto{-1.13}{4pt}}$&$5.46^{\scaleto{+0.11}{4pt}}_{\scaleto{-0.95}{4pt}}$&(5,12)\\
        22& PSOJ036+03 & 6.5405$\pm$0.0025 &\CII&$-27.33$&3.7$\pm$0.13&3.3$\pm$0.11&(6,9)\\
        \hline
        
        \multicolumn{8}{p{\linewidth}}{\small \textbf{Note.} References relate to redshift and magnitude respectively. (-) D'Odorico et al. (in prep); (1) Bischetti et al. (\citeyear{2022Natur.605..244B}); (2) Schindler et al. (\citeyear{2020ApJ...905...51S}); (3) Wang et al. (\citeyear{2010ApJ...714..699W}); (4) Carilli et al. (\citeyear{2010ApJ...714..834C}); (5) Decarli et al. (\citeyear{2018ApJ...854...97D}); (6) Venemans et al. (\citeyear{2020ApJ...904..130V}); (7) Jiang et al. (\citeyear{2007AJ....134.1150J}); (8) Wang et al. (\citeyear{2016MNRAS.460.2143W}); (9) Ba{\~n}ados et al. (\citeyear{2016ApJS..227...11B}); (10) Reed et al. (\citeyear{2017MNRAS.468.4702R});(11) Nanni et al. (\citeyear{Nannietal}); (12) Carnall et al, (\citeyear{2015MNRAS.451L..16C}).}
      \end{tabular}
      \caption{\label{tab:qso-rp}Proximity zone measurements: Columns show name of the quasar, redshift with error, emission line used for redshift, magnitude at 1450\AA, proximity zone size in proper Mpc with both redshift and continuum errrors, proximity zone corrected to $M_{1450}=-27.0$ in proper Mpc with both redshift and continuum errrors, and references for redshift and magnitude. \gk{Split this table into two.  This table should only list received data; the second table shoud list our contribution, i.e., proximity zone sizes.  Place the second table somewhere near Section 3.1.} \gk{When you split the table into two, there will be more space.  Use it to list the references directly in the table instead of the footnote.}}

    \end{table*}
  \end{center}
\end{comment}

\begin{comment}
  \multicolumn{2}{p{0.2\linewidth}}{\;\;Continuum errors ($\Delta\rp$)}
  \begin{center}
    \begin{table}
      \centering
      \begin{tabular} {p{0.05\textwidth} p{0.16\textwidth} p{0.12\textwidth} p{0.1\textwidth}}
	\hline
	\hline 
	S. No & Object & $\rp$ & $\rpc$ \\
	&            & (pMpc)  & (pMpc) \\
	\hline
	1 & J0408-5632  & $3.00^{\scaleto{+0.66}{4pt}}_{\scaleto{-0.37}{4pt}}$ &$3.5^{\scaleto{+0.76}{4pt}}_{\scaleto{-0.43}{4pt}}$ \\ 
	%\hline
	
	2 & PSOJ029-29 & $4.91^{\scaleto{+0.66}{4pt}}_{\scaleto{-0.37}{4pt}}$ &$4.4^{\scaleto{+0.59}{4pt}}_{\scaleto{-0.33}{4pt}}$ \\ 
	
	%\hline
	3 &ATLASJ029-36 &$4.33^{\scaleto{+0.65}{4pt}}_{\scaleto{-0.37}{4pt}}$&$4.34^{\scaleto{+0.65}{4pt}}_{\scaleto{-0.37}{4pt}}$\\
	
	%\hline
	4&VDESJ0224-4711&$6.45^{\scaleto{+0.59}{4pt}}_{\scaleto{-0.35}{4pt}}$&$6.61^{\scaleto{+0.6}{4pt}}_{\scaleto{-0.35}{4pt}}$\\
	
	%\hline
	5&PSOJ060+24* & $4.13^{\scaleto{+0.63}{4pt}}_{\scaleto{-0.35}{4pt}}$&$4.2^{\scaleto{+0.65}{4pt}}_{\scaleto{-0.36}{4pt}}$\\
	
	%\hline
	6&PSOJ108+08  &$1.99^{\scaleto{+0.14}{4pt}}_{\scaleto{-0.46}{4pt}}$&$1.63^{\scaleto{+0.12}{4pt}}_{\scaleto{-0.37}{4pt}}$\\
	%\hline
	
	7&SDSSJ0842+1218 & 6.89$\pm$0.14& 7.11$\pm$0.15\\
	%\hline
	
	8&PSOJ158-14* & 1.95$\pm$0.14&1.63$\pm$0.12\\
	%\hline
	
	9&PSOJ183-12&$3.06^{\scaleto{+0.67}{4pt}}_{\scaleto{-0.38}{4pt}}$&$2.58^{\scaleto{+0.57}{4pt}}_{\scaleto{-0.32}{4pt}}$ \\
	%\hline
	
	10&	PSOJ217-16 & $2.88^{\scaleto{+0.14}{4pt}}_{\scaleto{-0.6}{4pt}}$&$2.94^{\scaleto{+0.14}{4pt}}_{\scaleto{-0.61}{4pt}}$ \\
	%\hline
	
	11&	PSOJ242-12 &4.87$\pm$0.15&5.01$\pm$0.15\\
	%\hline
	
	12&	PSOJ308-27  &$2.95^{\scaleto{+0.68}{4pt}}_{\scaleto{-0.38}{4pt}}$&$3.19^{\scaleto{+0.74}{4pt}}_{\scaleto{-0.41}{4pt}}$ \\
	%\hline
	
	13&	PSOJ323+12* &6.2$\pm$0.13&5.95$\pm$0.12 \\
	%\hline
	
	14&	PSOJ359-06*  &2.71$\pm$0.14&2.92$\pm$ 0.15\\
	
	15&	SDSSJ0927+2001* &4.7$\pm$0.15&5.1 $\pm$0.16\\
	
	16&	SDSSJ0818+1722* &$5.13^{\scaleto{+1.43}{4pt}}_{\scaleto{-2.35}{4pt}}$ &$4.29^{\scaleto{+1.2}{4pt}}_{\scaleto{-1.96}{4pt}}$\\
	
	17&	SDSSJ1306+0356 & $6.43^{\scaleto{+0.14}{4pt}}_{\scaleto{-0.15}{4pt}}$&6.21$\pm$0.14\\
	
	18&	ULASJ1319+0950* & $3.87^{\scaleto{+1.08}{4pt}}_{\scaleto{-0.14}{4pt}}$&$3.81^{\scaleto{+1.07}{4pt}}_{\scaleto{-0.14}{4pt}}$\\
	
	19&	SDSSJ1030+0524* &$5.47^{\scaleto{+0.61}{4pt}}_{\scaleto{-0.34}{4pt}}$&$5.49^{\scaleto{+0.61}{4pt}}_{\scaleto{-0.35}{4pt}}$\\
	
	20&	SDSSJ0100+2802*&$7.22^{\scaleto{+0.13}{4pt}}_{\scaleto{-0.14}{4pt}}$&$3.43^{\scaleto{+0.06}{4pt}}_{\scaleto{-0.07}{4pt}}$\\
	
	21&	ATLASJ025-33&$6.5^{\scaleto{+0.14}{4pt}}_{\scaleto{-1.13}{4pt}}$&$5.46^{\scaleto{+0.11}{4pt}}_{\scaleto{-0.95}{4pt}}$\\
	
	22&	PSOJ036+03* &3.7$\pm$0.13&3.3$\pm$0.11\\
	\hline
	
	\multicolumn{4}{p{\linewidth}}{\small * refers to measurements that have been updated in this work.}
      \end{tabular}
      \caption{\label{tab:qso-rp}Proximity zone measurements: Columns show name of the quasar, proximity zone size in proper Mpc with both redshift and continuum errrors and proximity zone corrected to $M_{1450}=-27.0$ in proper Mpc with both redshift and continuum errrors. \gk{Can we add continuum error and redshift error and total error in three columns?  Since you have done the continuum error propagation for the first time, we should highlight it.}}
    \end{table}
  \end{center}
\end{comment}


